DarkHorse: A UDP-based Framework to Improve the Latency of Tor Onion Services

Tor is the most popular anonymous communication overlay network which hides clients' identities from servers by passing packets through multiple relays. To provide anonymity to both clients and servers, Tor onion services were introduced by increasing the number of relays between a client and a server. Because of the limited bandwidth of Tor relays, large numbers of users, and multiple layers of encryption at relays, onion services suffer from high end-to-end latency and low data transfer rates, which degrade user experiences, making onion services unsuitable for latency-sensitive applications. In this paper, we present a UDP-based framework, called DarkHorse, that improves the end-to-end latency and the data transfer overhead of Tor onion services by exploiting the connectionless nature of UDP. Our evaluation results demonstrate that DarkHorse is up to 3.62x faster than regular TCP-based Tor onion services and reduces the Tor network overhead by up to 47%.

==> sections/threat.tex <==
\section{Threat Model}
\label{sec:threat}

==> sections/use-cases.tex <==
\section{Use Cases and Motivation}
\label{sec:use-cases}
